Quantum Advantage with Faulty Oracle

This paper investigates the impact of noise in the quantum query model, a fundamental framework for quantum algorithms. We focus on the scenario where the oracle is subject to non-unitary (or irreversible) noise, specifically under the \textit{faulty oracle} model, where the oracle fails with a constant probability and acts as identity. Regev and Schiff (ICALP'08) showed that quantum advantage is lost for the search problem under this noise model. Our main result shows that every quantum query algorithm can be made robust in this noise model with a roughly quadratic blow-up in query complexity, thereby preserving quantum speedup for all problems where the quantum advantage is super-cubic. This is the first non-trivial robustification of quantum query algorithms against an oracle that is noisy.

==> grover-error-corrected.tex <==
\section{Grover error corrected}
We will show how to achieve the lower bound on on Grover search with a bit stronger oracle. We will have the addition oracle $\hat A^{k,(m)}:$\davidcom{I am not really happy that I have to give additional power to the oracle. However, while we can implement this oracle with two accesses of the oracle, I do not see a way to do it while maintaining our current error model.}

$$\hat A^{k,(m)} \ket{i}\ket{b} =\begin{cases}
    \ket{i}\ket{b+1 \mod m} & \text{if } i=k\\
    \ket{i}\ket{b} & \text{if } i\neq k\\
\end{cases}$$
and you are given a noisy version of this oracle:
$$A^{k,(m)}_p = (1-p)\hat A^{k,(m)} + p \mathrm{Id}$$

This is shown in $2$ steps. First we show how to implement the replacement oracle
$$O^{k,1/r} = e^{i\frac{\pi}{r}}\ketbra{k} + \sum_{i\neq k} \ketbra{i}$$
which has the analogous noisy version
$$O^{k,1/r}_p = (1-p)\hat O^{k,1/r} + p\cdot \mathrm{Id}$$
using only a single application of the oracle $A^{k,(r)}_p$.

Secondly, we will show that the oracle $\left(O^{k,O\left(\frac{1-p}{p\sqrt{N}}\right)}_p\right)^{O\left(\frac{p\sqrt{N}}{1-p}\right)}$ can used as a replacement of $\hat O^k$ without too much additional error in Grover's search algorithm. If this is true, then we observe that we need $O(p\sqrt{N}/(1-p)\cdot \sqrt{N}) = O(\frac{p}{1-p}N)$ applications of the oracle, which asymptotically achieves the lower bound for all values $p$.

We start with step $1$.

\begin{lemma}
    Given access to the oracle $A^{k,(2r)}_p$, then
    $$O^{k,1/r}_p(\ket{\phi}) = \tr_2(A^{k,(2r)}_p(\ket{\phi} \tensor \ket{\psi}))$$
    for the state $\ket{\psi} = \sum_{j=0}^{2r-1}e^{-i\frac{\pi j}{r}}\ket{j}$.
\end{lemma}
\begin{proof}
    %From the oracle $O^k$, before the algorithm, we use a single aplications to see check if $k=1$. If it is, then we are finished. So we can assume it isn't. Then observe that we now can implement a controlled version of $O^k_p$ by preparing $\ketbra{1}$ in an ancillary register, and swap this with the register that $O^k_p$ is being applied on, controlled by the control qbit.

    %Next, it is well known that applying a Hadamard gate $H$ before using the control qbit, we can construct a classical oracle $\hat O^k_c$. Finally, applying the classical oracle to the (unnormalised)state:
    %$$O^k_c\ket{k}(\ket{0} + e^{-i\frac{\pi}{r}}\ket{1}) = \ket{k}(\ket{0} + e^{-i\frac{\pi}{r}}\ket{1})$$
    Simply check that the addition shifts the basis vectors of $\ket{\psi}$ by one, giving a global phase of $e^{i\frac{\pi}{r}}$ when $\ket{\phi}=\ket{k}$ and no global phase otherwise.
\end{proof}

The idea now is that given the oracle $O^{k,1/r}_p$, with probability $p$ nothing happens. By applying this oracle $\frac{r}{p-1}$ times in succession, in expectation we would have applied the oracle $\hat O^{k}$. From the way we have constructed the oracle $O^{k,1/r}_p$, we are however going to be a bit of. This will however correspond to a small angle, which magnitude is dependent on the parameter $r$. We are going to give a bound on the parameter $r$.

\begin{lemma}\label{lem:angle-approx-error}
    For any angle $\theta\in \mathbb{R}$, $\left|e^{i\theta}+1\right|\le |\theta-\pi|$
\end{lemma}
\begin{proof}
    \begin{align*}
        \left|e^{i\theta}+1\right| &= |(\cos\theta + 1) + i\sin\theta|\\
        &= \sqrt{2 + 2\cos\theta}\\
        &\le \sqrt{2+2\left(\frac{(\theta-\pi)^2}{2}-1\right)}\\
        &= |\theta-\pi|
    \end{align*}
    using that $\frac{(\theta-\pi)^2}{2}-1\ge \cos\theta$. \davidcom{Probably need to be expanded a bit}
\end{proof}
Next, let $\ket{\eta} = \frac{1}{\sqrt{N}}\sum_{i=0}{N-1}\ket{i}$ and let $U_\eta = 2\ketbra{\eta}-I$. Then Grover's algorithm is the operator $U_\eta\hat O^{k}$ repeated $O(\sqrt{N})$ times on the state $\ket{\eta}$. We are not going to be able to exactly apply $\hat O^{k}$, but something that is close. Next we are going to show a central lemma, that allows us to average out this error:
\begin{lemma}\label{lem:operator-norm-swap}
    $$\norm{U_\eta O^{k,1/r}-O^{k,1/r}U_\eta}=O\left(\frac{1}{r\sqrt{N}}\right)$$
    Where the norm is the operator norm.
\end{lemma}
\begin{proof}
    Let $\ket{\eta'} = \frac{1}{\sqrt{N-1}}\left(\sqrt{N}\ket{\eta}-\ket{k}\right)$. It is clear that $\ket{\eta'}$ and $\ket{k}$ are orthogonal unitvectors, and that the actions of $U_\eta$ and $O^{k,1/r}$ can both be described in the basis $\{\ket{k},\ket{\eta'}\}$. In this basis we have
    $$\ket{k} = \left[\begin{matrix}1\\0\end{matrix}\right]$$
    $$\ket{\eta} = \frac{1}{\sqrt{N}}\left[\begin{matrix}1\\\sqrt{N - 1}\end{matrix}\right]$$
    $$O^{k,1/r}=\left[\begin{matrix}- e^{- i \frac{\pi}{r}} & 0\\0 & 1\end{matrix}\right]$$
    $$U_\eta = \left[\begin{matrix}-1 + \frac{2}{N} & \frac{2 \sqrt{N - 1}}{N}\\\frac{2 \sqrt{N - 1}}{N} & -1 + \frac{2 \left(N - 1\right)}{N}\end{matrix}\right]$$
    $$U_\eta O^{k,1/r}-O^{k,1/r}U_\eta = \frac{1}{N}\left[\begin{matrix}0 & 2 \sqrt{N - 1} \left(e^{\frac{i \pi}{r}} + 1\right) e^{- \frac{i \pi}{r}}\\- 2 \sqrt{N - 1} \left(e^{\frac{i \pi}{r}} + 1\right) e^{- \frac{i \pi}{r}} & 0\end{matrix}\right]$$
    Finally, 
    $$\norm{U_\eta O^{k,1/r}-O^{k,1/r}U_\eta}=2 \left|{\frac{\sqrt{- \left(N - 1\right) e^{- 2 i \frac{\pi}{r}}} \left(e^{i \frac{\pi}{r}} + 1\right)}{N}}\right|=O\left(\frac{1}{r\sqrt{N}}\right)$$
    using \cref{lem:angle-approx-error}.\davidcom{Done using CAS tools}
\end{proof}
What this lemma shows is that we can essentially swap a $O^{k,1/r}$ and a $U_\eta$ and accumulate way less error compared to simply removing the $O^{k,1/r}$. This means that we essentially will be able to average out the inaccuracies $O^{k,1/r}_p$ over all $\sqrt{N}$ of the applications of $O^{k}$, with a bit of additional error, instead of having to do it individually for each application. Then it is just to calculate the expected error.

% \manaswicom{Hi David, your writeup looks quite interesting. Section 3 of this \href{https://arxiv.org/pdf/quant-ph/0304138}{paper} might be of interest. It is quite nice how the upper-bound of $O(pN/(1-p))$ can be achieved when $m$ is allowed to be $2r$ which can be as large as $(p/(1-p))\sqrt{N}$. It might be nice to think whether the matching upper bound of $O(pN/(1-p))$ can be achieved when $m$ is bounded. Recall that for Grover's algorithm $m = 2$, which is then used to obtain the phase oracle $\widehat{O}^k$. If an upper bound of $O(pN/(1-p))$ can not be achieved for small $m$ then, with your proof, perhaps we can say that extra ``space'' gives some advantage (given the setting in which we are working, I am not sure how we would formalize this). I have a question regarding interpretation of the last lemma (Lemma 1.3). It would be nicer to discuss this in person on 3rd July.}
% \davidcom{We actually only need $m=O(p\sqrt{N})$, since the $\frac{1}{(1-p)}$ is just to get the correct mean.}
% \manaswicom{Another vague question, more of a note-to-self, is that having $m = O(\sqrt{N})$ suffices, for constant $p$. Extra ``space'' does not give additional advantage (due to lower bound). Is there a connection to query complexity or query depth?}

\begin{lemma}\label{lem:Si-step-bound}
    Let 
    $$S_i = ((O^{k,1/r})^{X_{\sqrt{N}}}U_\eta)((O^{k,1/r})^{X_{\sqrt{N}-1}}U_\eta)\cdots((O^{k,1/r})^{X_{i+1}}U_\eta)((O^{k,1/r})^{Y_{i}}U_\eta)(O^{k}U_\eta)^{i-1}$$
    where $X_i$ is the random variable denoting the number of times $O^{k,1/r}$ was applied in the $i'$th round and $Y_i=\sum_{j\le i} X_i-(i-1)r$. Then 
    $$E[\norm{S_{i+1}-S_i}] = O\left(\sqrt{\frac{ip}{rN}}\right)$$
    where the norm is the 
\end{lemma}
\begin{proof}
    Observe that $S_i$ and $S_{i+1}$ only differ on the $i$ and $i+1$ set of operators. Therefore we can bound the difference by:
    
    $$\norm{S_{i+1}-S_{i}}\le \norm{(O^{k,1/r})^{X_{i+1}}U_\eta(O^{k,1/r})^{Y_{i}}-(O^{k,1/r})^{Y_{i+1}}U_\eta O^{k}}.$$
    Next we observe that
    $$(O^{k,1/r})^{Y_{i+1}}U_\eta O^{k} = (O^{k,1/r})^{X_{i+1}}(O^{k,1/r})^{Y_{i}-r}U_\eta O^{k}$$
    implying 
    $$\norm{(O^{k,1/r})^{X_{i+1}}U_\eta(O^{k,1/r})^{Y_{i}}-(O^{k,1/r})^{Y_{i+1}}U_\eta O^{k}} = \norm{U_\eta(O^{k,1/r})^{Y_{i}-r}-(O^{k,1/r})^{Y_{i}-r}U_\eta}$$
    while also using that $(O^{k,1/r})^{r} = O^{k}$. This directly gives us that the operator norm is bounded by $|Y_i-r|$ applications of \cref{lem:operator-norm-swap}. This means that 
    $$\norm{S_{i+1}-S_{i}} = O\left(\frac{|Y_i-r|}{r\sqrt{N}}\right)$$

    Next we observe that the random variable is distributed like $Y_i+(i-1)r\sim \mathrm{Bin}(ir/(1-p),p)$ and has mean $ir$. This means that we can write
    $E[|Y_i-r|] = E[|(Y_i + (i-1)r)-ir|]$
    which is upper bounded by the standard deviation of $Y_i+(i-1)r$, giving
    $$E[|Y_i-r|] \le \sqrt{\frac{ir}{1-p}p(1-p)}=\sqrt{irp}$$
    This directly gives us that
    $$E[\norm{S_{i+1}-S_i}] = O\left(\frac{\sqrt{irp}}{r\sqrt{N}}\right)=O\left(\sqrt{\frac{ip}{rN}}\right)$$
\end{proof}

\begin{theorem}
    When $r=\Omega(\sqrt{N}p)$, $E[\norm{S_{\sqrt{n}}-S_1}]\le \frac{1}{3}$.
\end{theorem}
\begin{proof}
    By the triangle inequality, we have
    $$\norm{S_{\sqrt{N}}-S_1} \le \sum_{i=1}^{\sqrt{N}-1}\norm{S_{i+1}-S_i} =\sum_{i=1}^{\sqrt{n}-1} O\left(\sqrt{\frac{ip}{rN}}\right)$$
    Using that $\sum_{i=1}^{n}\sqrt{i} = O(n^{3/2})$, we get
   $$\norm{S_{\sqrt{n}}-S_1} =O\left(\sqrt{\frac{p}{r}}N^{1/4}\right)$$
    Requiring $\norm{S_{\sqrt{n}}-S_1}\le \frac{1}{3}$ implies 
    $r=\Omega(p\sqrt{N})$
\end{proof}
Note that $S_{\sqrt{n}}$ corresponds to Grover search while $S_1$ corresponds to the noisy version of Grover search. Furthermore, this bound gives us that since we have used $\frac{r}{(1-p)}\sqrt{N}$ applications of the oracle, we have in total used $O(\frac{p}{p-1}N)$ applications of the oracle which corresponds to the lower bound.

\section{A different approach that works in all the error models}
%\label{sec: A different approach that works in all the error models}
We use the following approach. Assume that $(1-p)=\Omega(1)$. Run $1/p$ iterations of Grovers algorithm then measure.

The probability of the Oracle never failing can be found as 
$$\left(1-p\right)^{1/p} = O(1)$$
Using that $1-p$ is a constant.

The probability of Grover's algorithm succeeding after $r$ iterations can be found as
$$s = \sin^2\left(2\left(\frac{1}{2}+r\right)\sin^{-1}(\frac{1}{\sqrt{N}})\right)$$
I will use the following two approximations. First, there exists constants $c_1,c_2$ such that
$$c_1\theta \le \sin\theta \le c_2\theta$$
for all $c_1,c_2\in [0,\pi]$ and $\sin$ is monotonically increasing in this interval. Secondly, there exists constants $d_1,d_2$ such that
$$d_1\theta \le \sin^{-1}\theta \le d_2\theta$$

We will now calculate the probability of Grovers algorithm succeeding after $1/p$ iterations:
\begin{align*}
    \sin^2\left(2\left(\frac{1}{2}+\frac{1}{p}\right)\sin^{-1}\left(\frac{1}{\sqrt{N}}\right)\right) &\ge\sin^2\left(2\left(\frac{1}{2}+\frac{1}{p}\right)\frac{d_1}{\sqrt{N}}\right)\\
    &= \sin^2\left(\frac{d_1}{\sqrt{N}} + \frac{d_1}{p\sqrt{N}}\right)\\
    & \ge \left(\frac{c_1d_1}{p\sqrt{N}}\right)^2\\
    &= \Omega\left(\frac{1}{p^2 N}\right)
\end{align*}
So from this we conclude that we should make $O(p^2N)$ parallel repetitions of Grovers algorithms to achieve constant probability of success. This gives $\Theta(pN)=\Theta(\frac{pN}{(1-p})$ total applications of the oracle.



\section{Bounds for Classical Noisy Oracle}

Consider a noisy classical oracle access to  $(x_1, \dots, x_n) \in \{0,1\}^n$ such that independently for all $i \in n$,
\begin{align*}
    \Pr[\text{the oracle returns } 1 \text{ upon querying } i \mid x_i = 1] &= \alpha \\
    \Pr[\text{the oracle returns } 1 \text{ upon querying } i \mid x_i = 0] &= 0.
\end{align*}


Our goal is to compute $\OR_n(x)$ for all $x \in \{0,1\}^n$, with error probability at most $1/10$, given access to such an oracle for $x$. We give a query complexity of $\Theta(n/\alpha)$.

\paragraph{Upper Bound.} Consider the following algorithm:
\begin{enumerate}

    \item For each $i \in S$, query $x_i$ $O(1/\alpha)$ many times. If a $1$ is observed, return $1$

    \item Else return $0$
\end{enumerate}

The number of queries made by the above algorithm in the worst case is $O(n/\alpha)$. Next, we analyze the correctness probability. First, if $x = 0^n$, then the algorithm makes no error. Thus let $x \neq 0^n$ and let $x_i = 1$ for some $i \in [n]$. Probability that $1$ is observed when $i$ is queried in Step 2. is at least $9/10$ for a (suitable choice of constant).



\paragraph{Lower Bound.} Let $A$ be a deterministic algorithm that makes $T$ queries and distinguishes $0^n$ and a random string of Hamming weight $1$, with error at most $1/10$.
Due to symmetry, we assume that the algorithm queries the indices $1, \dots, T$, and obtains bits $b_1, \dots, b_T$. If $x = 0^n$ then each of these bits are $0$, thus we consider the case when $x$ is a random string of Hamming weight $1$. In this case, we have $\Pr[b_i = 1] = \alpha/n$ for all $i \in [T]$. 
We have
\begin{align*}
    \Pr[b_1 = 0, \dots, b_T = 0]
    &= \prod_{k = 1}^T \Pr[b_k = 0 \mid \cap_{j = 1}^{k-1} b_j = 0] \\
    &= \prod_{k = 1}^T \left( 1- \frac{\alpha}{n-k+1} \right) \\
    &\geq (1 - \alpha/n)^T \geq 1 - (\alpha T)/n \label{eq: lb one-sided error classical OR}
\end{align*}
where in the last inequality we used $(1-x)^r \geq 1 - rx$ for $x \geq -1$ and $r \geq 1$.
Thus if $T \leq n/(100 \alpha)$ then with probability at least $99/100$, the algorithm sees all $0$'s and can not be correct with error probability at most $1/10$.

Another way to think about the above inequalities is that in the independent case algorithm is sampling with  replacement, in which the lower bound of $99/100$ is easy to see. Non-independent case is that of sampling without replacement, in which case the probability of seeing a $1$ increases every time a $0$ is sampled (when $x$ is a string of non-zero Hamming weight).

{\color{brown}\textbf{Manaswi:} We can also consider the more general model:
\begin{align*}
    \Pr[\text{the oracle returns correct answer} \text{ upon querying } i] \geq 1/2 + \delta.
\end{align*}
For this model $\Theta(n/\delta^2)$ should be tight for classical with same error as above.
}

\section{Questions}
\begin{itemize}
    \item Let $x \in \{0,1\}^n$ be unknown and consider the task of learning $x$ exactly and with high probability under various query models. If we can learn efficiently under some model, then we can compute any function. In particular, say a function has quantum query complexity $\Theta(n)$, like parity, majority and most functions, then a simple algorithm to compute such a function is to learn $x$.
    
    Given an oracle that makes no error, $n$ queries are necessary and sufficient to learn $x$. In~\cite{buhrman2007robust}, it was shown that under reversible noise (i.e. given access to a unitary and its inverse that produces noise), any string can be learnt using $O(n)$ queries. Is it interesting to ask this question for other noise models?

    
\end{itemize}

==> introduction_old.tex <==
\section{Introduction}

Understanding and mitigating noise is one of the most important challenges in quantum computing today and the quantum query model is one of the most natural models of computation to study the effects of noise.
% In this model, the goal is to decide whether an unknown function $f :\{0,1\}^n \to \{0,1\}$ satisfies some fixed property, when the function can only be accessed by a unitary matrix $O_f$, called \textit{oracle}, that satisfies $O_f \ket{z}\ket{b} = \ket{z} \ket{b \oplus f(x)}$ for all $x \in \{0,1\}^n$ and $b \in \{0,1\}$.
In this model, the goal is to compute a known function $g : \{0,1\}^n \to \{0,1\}^m$ on an unknown input $x \in \{0,1\}^n$. The input $x$ can only be accessed by a unitary matrix $O_x$, called \textit{oracle}, that satisfies $O_x \ket{i}\ket{b} = \ket{i} \ket{b \oplus x_k}$ for all $i \in \{1, \dots, n\}$ and $b \in \{0,1\}$, where $x_i$ denotes the $i$th bit of $x$ and $\oplus$ denotes XOR. 
Furthermore, the goal is to compute $g(x)$ for all $x \in \{0,1\}^n$ with bounded-error\footnote{By bounded-error we mean correctly with probability at least $4/5$. Algorithms that have success probability $(1/2 + \delta)$ can be made bounded-error by amplitude amplification~\cite{brassard2002quantum} with an overhead of $O(1/\delta)$.}. by making minimum number queries to $O_x$. 
Most of the provable advantages of quantum algorithms over classical ones are in this model (for example, Grover's algorithm for search (\cite{grover1996fast}) and Shor's Algorithm for period finding (\cite{shor1999polynomial})) and this model is naturally connected to many other areas of quantum computing due to its simplicity. Thus, understanding the effects of noise in the query model is a fundamental question. 


In this paper, we are interested in the case when the oracle is affected by noise\footnote{There has been work dealing with noise affecting other components of query algorithms (see~\cite{R03} and the references therein).}.
There are two types of noise that may affect the oracle: unitary (or reversible) and non-unitary (or irreversible). An example of a reversible noisy oracle is a low-depth quantum circuit implemented on a fault-tolerant quantum quantum computer. However, when such a circuit is implemented on a quantum computer that is not fault-tolerant and is affected by noise due to its interaction with the environment, we have an oracle with non-reversible noise.  The reversible noise is well-understood and easy to mitigate: a quantum algorithm designed for a fault-less oracle with cost $q$ can be easily modified to give an algorithm for a with cost $O(q \log q)$ that works correctly on an oracle with reversible noise (\cite{hoyer2003quantum, suzuki2006robust, buhrman2007robust, iwama2006query}).

Understanding non-reversible noise in the query model has proved much more challenging.
The majority of existing results are limited to the study of the effects %of various types of 
non-reversible noise for Grover's algorithm~\cite{PR99, LLZT00, SBW03, FG98, ABNR12, KNR18} or for the search problem itself~\cite{RS08, VRRW14, R03}.
To the best of our knowledge, search is the only problem for which lower bounds under a noisy oracle are known. The work~\cite{RS08} gave the first such lower bound under the following noise model: we are given access to a faulty oracle $O_{f,p}$ which acts as follows
% which with probability $p$ fails and acts as identity, while with probability $(1-p)$ acts as $O_f$
\begin{align*}
    O_{f,p}(\cdot) = \begin{cases}
    O_f(\cdot) & \text{ with probability $(1-p)$}\\
    I(\cdot) & \text{ with probability $p$}.
\end{cases} \tag*{(Faulty Oracle) \qquad}
% \label{eq: Intro Defn RS Noise}
\end{align*}
where $I$ is the identity map, i.e., $I(\rho) = \rho$ for all matrices $\rho$.
% Generally speaking, these papers show that if noise occurs at a large enough rate, then quantum advantage is lost for the search problem. We refer to~\cite{R03} for a survey of these results. A landmark result in this line of work was~\cite{RS08} which gave the first lower bound for the search problem under the following noise model: we are given access to an oracle $O_{f,p}$ which with probability $p$ fails and acts as identity, while with probability $(1-p)$ acts as $O_f$. 
Similar to~\cite{RS08}, we refer to this error model as the \textit{faulty oracle} model.
The parameter $p$ is called the error rate. The faulty oracle model, when the error rate $p$ is at most  $1/2$, is the central object of study in this paper. 
It is natural to consider the regime where the error-rate is a constant independent of the system size. This is what we focus on.

% It is natural to consider the regime where the error-rate is independent of the system size as we do not expect to be able to build larger quantum systems more reliably than smaller ones (so in practice the error rate should stay the same or increase with the size of the system, prior to error correction).
% \lauracom{I tried to rephrase.} 
%This range of error rate is perhaps the most natural to consider since we do not expect to build systems where the error-rate would scale down with the system size.}\davidcom{There is something weird in this sentence. If the error rate increases, this would correspond to $p$ increasing, which doesn't seem to correspond to what is being written} \manaswicom{I guess what I mean is that systems of larger size should have larger error, i.e. $p$ should be large. Thus error-rate should not scale down as size of system increases. Perhaps we should write this more clearly?}
% This noise model, specifically when $p = 1/2$, is the central object of study in this paper. 
% \davidcom{This makes it seem like we can only handle error of $p=1/2$. We should probably make it clear that it can be easily extended to $p\le 1/2$.} \manaswicom{Sure. I wanted to stress that our results hold for constant $p$. I have changed the last line.}

The work \cite{RS08} showed an $\Omega(pn)$ lower bound for the search problem in the faulty oracle model. This means that quantum advantage is lost when the error rate is a constant. This lower bound has impacted several areas of research in quantum computing.~\cite{AGJMP15} considered quantum random access memory (qRAM) that stores classical information, i.e.~bits. Such a qRAM can be used as an oracle for quantum query algorithms.~\cite{AGJMP15} defines an error model that is quite similar to the faulty oracle model. Using the lower bound of~\cite{RS08}, they showed that a qRAM that produces queries with constant error will not lead to a quantum advantage for the search problem. Furthermore,~\cite{AGJMP15} conjectured that their error model nullifies the asymptotic speed-ups of other quantum query algorithms as well.
% ~\cite{xu2023systems} emphasis that, in view of the lower bound of~\cite{RS08}, it is critical to guarantee the error robustness of qRAM, via either intrinsic noise resilience or error correction.
Most supervised quantum machine learning algorithms assume the existence of qRAM (\cite{GLM08}). In view of this and~\cite{RS08}, the authors of~\cite{wossnig2021quantum} suggested that even small errors can crucially impact quantum machine learning algorithms.~\cite{R03} studied the query complexity of the search problem under depolarizing noise and gave an $\Omega(np)$ lower bound for the search problem under this noise model.

A natural question to ask is whether there are problems for which a quantum advantage is retained even under a noisy oracle.

\begin{center}
    \textit{\textbf{Question.} Is there any reasonable fault model for which a quantum speed-up is achievable? (\cite{RS08}) Is a significant quantum speedup is ever possible with a faulty oracle? (\cite{childs2023streaming})}
\end{center}

If we restrict our attention to quantum algorithms where the (parallel) query depth is upper bounded by a constant, for example Simon's algorithm~\cite{simon1997power}, then the answer to the question is indeed yes (with a polynomial overhead) under the faulty oracle model.~\cite{childs2023streaming} studied the case when the oracle has depolarising noise. They showed that quantum algorithms with constant query depth can be made robust with a polynomial overhead. However, their techniques do not extend to algorithms that have $\omega(1)$ query depth without a substantial overhead. Prior to our work, there were no known techniques allowing one to maintain quantum advantage in the noisy regime beyond the case of constant (parallel) query depth.
% \manaswicom{Name the noise model as RS-Noisy Oracle? Define other noise models? TODO: Mention that we are dealing with constant error rate.} \davidcom{So far I have called the noise for ``faulty oracle'', but I am not sure if there is a better name for it}

The main contribution of this paper is to show that in the faulty oracle model, a quantum advantage is retained for \textit{every} quantum query algorithm that is sufficiently fast, in the regime of a constant error rate $p\leq 1/2$.
%(given this, the case when $p < 1/2$ follows trivially). 
In the next section, we present our main result which shows how to make a quantum algorithm robust to faulty oracle with a roughly quadratic blow-up in query complexity.
% Thus we answer the \textbf{Question.} is affirmative for the extensively studied faulty oracle model for \textit{all} quantum algorithms that are sufficiently fast\footnote{Mention quantitatively}. In the next section, we describe our main results.

\section{Our Results}

We state our main theorem informally, referring to \cref{sec:any-algorithm} for the formal discussion.

\begin{theorem}[\textbf{Informal}]
\label{thm: Informal Main Theorem}
    Consider any $f : \{0,1\}^n \to \{0,1\}^m$ and a bounded-error quantum query algorithm $\mathcal{A}$ that solves a problem $P$ by making $q$ queries to a (fault-free) oracle $O_f$. Then there exists a bounded-error quantum algorithm $\mathcal{A}'$ that solves $P$ and makes $O(q^3 m^2 \log q)$ queries to the faulty oracle $O_{f,p}$ where $p \leq 1/2$.
\end{theorem}

% \begin{theorem}[\textbf{Informal}]
% \label{thm: Informal Main Theorem}
%     Let $g : \cD \to \{0,1\}^m$, where $\cD \subseteq \{0,1\}^n$, such that there exists a bounded-error quantum query algorithm that computes $g(x)$ for all $x \in \cD$ by making at most $q$ queries to a fault-free oracle $O_x$. Then there exists a bounded-error quantum algorithm that computes $g(x)$ for all $x \in \cD$ by making $O(q^3 m^2 \log q)$ many queries to a faulty oracle $O_{x,p}$, with error-rate $p \leq 1/2$.
% \end{theorem}

% In particular, the query cost of a quantum algorithm for $f$ robust to noisy oracle is $O(Q(g)^3 \log Q(g))$, where $Q(g)$ is the quantum query complexity of $g$ (see Section~\ref{} of the full-version of the paper for the definition of query complexity).

While quantum advantage is lost for the search problem with a faulty oracle (\cite{RS08}), Theorem~\ref{thm: Informal Main Theorem} implies that a quantum advantage is retained for all problems for which there is a quantum algorithm with roughly super-cubic advantage. Furthermore, no additional structural assumptions are made about the algorithms, such as bounded-query depth as considered in~\cite{childs2023streaming}, in Theorem~\ref{thm: Informal Main Theorem}. There are several quantum query algorithms that have super-cubic, super-polynomial, and even exponential advantage over their classical counterparts, and from Theorem~\ref{thm: Informal Main Theorem}, a quantum advantage is retained for these algorithms. We refer the reader to~\cite{Zoo} which contains an extensive collection of such quantum algorithms.~\cite{RS08} asked the following question.
% \manaswicom{Include some algorithms not in this list.} \manaswicom{Include some algorithms from property testing.}


\begin{openproblem}[\cite{RS08}]
    Is there any search problem for which a quantum speed-up is achievable with a faulty oracle?
\end{openproblem}

Theorem~\ref{thm: Informal Main Theorem} resolves this problem in the affirmative when combined with the following search algorithms: super-polynomial speedup for the welded tree problem which involves finding a special vertex in a certain graph (\cite{childs2003exponential, li2024recovering, jeffery2023multidimensional, belovs2024global})
and \textit{quartic} speedup for searching counterfeit coins given a bunch of coins (\cite{iwama2012quantum}).

We conclude with some ideas that went into the proof of Theorem~\ref{thm: Informal Main Theorem}.

\begin{figure}[t]

\begin{minipage}[c]{0.35\linewidth}
    % \centering
        % \begin{quantikz}
        % % \ket{z}_Z&\gate[2]{F_f^t}& \\
        % \ket{0}_S&&
        % \end{quantikz}=
        \begin{quantikz}
        \ket{i}_Z&
        &\gate[2]{O_{f,\frac{1}{2}}}\gategroup[2,steps=2,style={rounded corners,dashed,inner sep=6pt, 
        % label = below:$F_x$
        },label style={label
position=above right,anchor=north,xshift=0.40cm,yshift=0cm}]{$\times t$} &  & & & \\
        \ket{0}_S & \gate{R_{-\pi/4}} &  & \gate{R_{\frac{\pi}{2t}}} &  & \gate{R_{-\pi/4}} &
        \end{quantikz}
\end{minipage} \qquad \qquad \qquad \qquad
\begin{minipage}[c]{0.3\linewidth}
        % \begin{quantikz}
        % \ket{z}_Z&\gate[3,nwires=2]{G_f^t}& \\
        % \setwiretype{n}&&\\
        % \ket{b}_B&&
        % \end{quantikz}=
        \begin{quantikz}
        \ket{i}_Z&\gategroup[3,steps=6,style={rounded corners,dashed,inner sep=6pt, }]{} & \gate[2]{F_f^t} & & & \gate[2]{F_f^t} & & \\
        \setwiretype{n}&\ket{0}_S&\setwiretype{q} & \ctrl{1} & \gate{X} &  & \gate{X} &\\
        \ket{b}_B&&&\targ{}&&&&
        \end{quantikz}
\end{minipage}
\caption{The circuit to the left is $F_f^t$ and the  circuit to right is $G_f^t$.} 
\label{fig: intro figure}
\end{figure}


% \begin{figure}[t]
%     \centering
%         \begin{quantikz}
%         \ket{z}_Z&\gate[2]{F_f^t}& \\
%         \ket{0}_S&&
%         \end{quantikz}=\begin{quantikz}
%         \ket{z}_Z&
%         &\gate[2]{O_{f,\frac{1}{2}}}\gategroup[2,steps=2,style={rounded corners,dashed,inner sep=6pt, },label style={label
% position=above right,anchor=north,xshift=0.40cm,yshift=0cm}]{$\times t$} &  & & & \\
%         \ket{0}_S & \gate{R_{-\pi/4}} &  & \gate{R_{\frac{\pi}{2t}}} &  & \gate{R_{-\pi/4}} &
%         \end{quantikz}
%     \caption{Robust calculation of $O_{f}\ket{z,0}$}
%     \label{alg:robust-0-oracle}
% \end{figure}



% \begin{figure}[t]
%     \centering
%         \begin{quantikz}
%         \ket{z}_Z&\gate[3,nwires=2]{G_f^t}& \\
%         \setwiretype{n}&&\\
%         \ket{b}_B&&
%         \end{quantikz}=\begin{quantikz}
%         \ket{z}_Z&\gategroup[3,steps=6,style={rounded corners,dashed,inner sep=6pt, }]{} & \gate[2]{F_f^t} & & & \gate[2]{F_f^t} & & \\
%         \setwiretype{n}&\ket{0}_S&\setwiretype{q} & \ctrl{1} & \gate{X} &  & \gate{X} &\\
%         \ket{b}_B&&&\targ{}&&&&
%         \end{quantikz}
%     \caption{Robust calculation of $O_{f}\ket{z,b}$}
%     \label{alg:robust-full-oracle}
% \end{figure}

\subsection{Ideas behind proof of Theorem~\ref{thm: Informal Main Theorem}}

We present our ideas when $\cD = \{0,1\}^n$ and $m = 2$, i.e.~when $g$ has domain $\{0,1\}^n$ and range $\{0,1\}$. The proof for a general $m$ follows from this case along with a careful error-analysis. Let $\cA$ be an algorithm that makes at most $q$ queries to the fault-less oracle $O_x$ and computes $g(x)$ correctly for all $x \in \{0,1\}^n$ with bounded-error. Such an algorithm uses three registers: $Z$ which stores the index to the query, $B$ which stores the output of the query, and $T$ which is the work-space used by the algorithm. Let 
$$
\cA = U_q (O_x\otimes I_T) U_{q-1} (O_x\otimes I_T) \ldots U_1 (O_x\otimes I_T)U_0
$$
% \begin{align*}
%     \cA = U_q (O_x\otimes I_T) U_{q-1} (O_x\otimes I_T) \ldots U_1 (O_x\otimes I_T)U_0
% \end{align*}
where $U_i'$'s act on $Z,B$ and $T$ while $O_x$ acts on $Z$ and $B$. The robust version of $\cA'$ uses an additional register $S$ (called scratch-pad) and is of the form
$$
\cA' = (U_q\otimes I_S)  (G_x^t\otimes I_T) \ldots (U_1\otimes I_S) (G_x^t\otimes I_T)
$$
% \begin{align*}
%     \cA' = (U_q\otimes I_S)  (G_x^t\otimes I_T) \ldots (U_1\otimes I_S) (G_x^t\otimes I_T)
% \end{align*}
where $U_i$'s act as identity on $S$, $t = O(q^3 \log q)$, and  $G_x^t$ act as identity on the work-space $T$. The unitaries $G_x^t$ are constructed from $O_{x,p}$ as shown in Figure~\ref{fig: intro figure}.
With high probability over the randomness of $O_{x,p}$, $G_x^t$
satisfy the following property: for a suitable choice of $t = O(q^2 \log q)$ and for all $\ket{\psi} \in \mathbb{C}^{Z + B + T}$ 
$$
\norm{((O_x\otimes I_{ST})-(G_x^t\otimes I_T))\ket{\psi}\ket{0}_S} \leq O(1/q).
$$
By an application of triangle inequality and discarding the scratch-pad registers at the end of the computation, the algorithm $\cA$ and $\cA'$ are close to each other on all inputs. Thus, at an overhead of $O(q^2 \log q)$, we show how to make a $q$-query bounded-error quantum algorithm robust to a faulty oracle. Observe that this error reduction procedure does not depend on the algorithm $\cA$.

The construction of $G_x^t$ can be broken down into two steps. First, consider the circuit $F_x^t$ shown in Figure~\ref{fig: intro figure}. We show that if the output register $B$ is in the state $\ket{0}$ then, with high probability, $F_x^t$ acts almost identically to $O_x$. Since $O_{x,p}$ acts as $I$ when $x_i = 0$ for all $p$, this case is easy to analyze. When $x_i = 1$, then for $p = 1/2$, the action of this circuit can seen as an unbiased random walk in a two-dimensional plane. We show that $t = O(q^2 \log q)$ repetitions of $F_x$ achieve sufficient concentration for the underlying random walk. This circuit acts close to $O_x$ when $B$ is in the state $\ket{0}$. We remove this restriction in the next step where we then extend the circuit $F_f^t$ to the circuit $G_f^t$, where we follow the standard technique of using $F_f^t$ to compute the state $\ket{f(i)}$, use this for a $CNOT$ gate and then finally uncompute the $\ket{f(i)}$ using $F_f^t$ again.

% \begin{itemize}
%     \item Consider the circuit $F_x^t$ shown in Figure~\ref{fig: intro figure}. We show that if the register $B$ is in the state $\ket{0}$ then $F_x^t$ acts almost identically to $O_x$, with high probability. Since $O_{x,p}$ acts as $I$ when $x_i = 0$ for all $p$, this case is easy to analyze. When $x_i = 1$, then for $p = 1/2$, the action of this circuit can seen as an unbiased random walk in a two-dimensional plane. We show that $t = O(q^2 \log q)$ receptions of $F_x$ achieves achieves sufficient for the underlying random walk. This circuit acts close to $O_x$ when $B$ is the state $\ket{0}$. We remove this restriction in the next step.

%     \item Next, we then extend the circuit $F_f^t$ to the circuit $G_f^t$ \manaswicom{@David: Couple of line intuition of $G_x^t$?}
% \end{itemize}

% We are going to be proving this in $4$ steps. First  in \cref{sec:boolean-functions} we are going to construct a circuit $F_f^t$, seen in \cref{alg:robust-0-oracle} that when given a $\ket{0}$ in the output register acts almost identically to $O_f$. 
% We are able to do this by creating a circuit that for a state $\ket{z,0}$ rotates the state by a small angle $\frac{\pi}{2t}$ whenever $f(z)=0$ and acts very similar to an unbiased random walk when $f(z)=1$. By repeating this circuit $t$ times we then get for large enough $t$ that the random walk achieves sufficient concentration in how much it has moved.

% Next in \cref{sec:full-oracle-replacement} we then extend the circuit $F_f^t$ to the circuit $G_f^t$, seen in \cref{alg:robust-full-oracle}. $F_f^t$ is fairly limited in which states it acts correctly on. However we can by using an additional register as a scratchpad implement $G_f^t$ which acts almost identically to $O_f$, though with some probability of error and a distance that can be made arbitrarily small by increasing $t$.

% In \cref{sec:multi-bit-functions} we discuss extending the circuit to be able to handle functions $f : \{0,1\}^n\to \{0,1\}^m$, the results of which can be seen in \cref{alg:robust-0-oracle-multi} and \cref{alg:robust-full-oracle-multi} This ends up being reasonably simple, as we can run the single-bit error correction $m$ times in parallel for every single output bit.

% Finally, in \cref{sec:any-algorithm} we show that using our replacement oracle we can for any algorithm that uses $q$ queries to the oracle $O_f$ implement this algorithm such that it with constant probability gets within a constant distance using $O(q^3\lg q)$ queries to the $O_{f,p}$ oracle.

% \begin{align*}
%     \norm{((O_x\otimes I_{ST})-(G_x^t\otimes I_T))\ket{\psi}_{ZBT}\ket{0^m}_S} \leq 1/(10q).
% \end{align*}
% $\norm{((O_f\otimes I_{ST})-(G_f^t\otimes I_T))\ket{\psi}_{ZBT}\ket{0^m}_S} = O(1/q)$.
% \begin{itemize}
%     \item They act as identitu
% \end{itemize}






% We are going to be proving this in $4$ steps. First  in \cref{sec:boolean-functions} we are going to construct a circuit $F_f^t$, seen in \cref{alg:robust-0-oracle} that when given a $\ket{0}$ in the output register acts almost identically to $O_f$. We are able to do this by creating a circuit that for a state $\ket{z,0}$ rotates the state by a small angle $\frac{\pi}{2t}$ whenever $f(z)=0$ and acts very similar to an unbiased random walk when $f(z)=1$. By repeating this circuit $t$ times we then get for large enough $t$ that the random walk achieves sufficient concentration in how much it has moved.

% Next in \cref{sec:full-oracle-replacement} we then extend the circuit $F_f^t$ to the circuit $G_f^t$, seen in \cref{alg:robust-full-oracle}. $F_f^t$ is fairly limited in which states it acts correctly on. However we can by using an additional register as a scratchpad implement $G_f^t$ which acts almost identically to $O_f$, though with some probability of error and a distance that can be made arbitrarily small by increasing $t$.




% \manaswicom{Perhaps the theorems also hold for partial functions, i.e. functions with domain $D \subseteq \{0,1\}^n$. We could state the main theorem for such functions and say that the proof naturally extends to such functions. Writing in this manner is important as exponential quantum advantage is possible for partial functions.}

% \manaswicom{Another nice thing to mention, if easily doable, is the blowup in the circuit size in the error-reduction in terms of the circuit size of the error free case.}

% \manaswicom{For Boolean valued function $S$ is a one-qubit register. Do we add one qubit to $S$ each time we make query?}

% \manaswicom{The circuit diagram of $F_f^t$ should have the register $B$ also? Since the oracle acts on $B$?}

==> introduction_old_old.tex <==
\section{Introduction}
Understanding and mitigation noise is one of the most important challenges in quantum computing today and the quantum query model is one of the most natural models of computation to study the effects of noise. In this model, the goal is to compute a known function $g : \{0,1\}^n \to \{0,1\}^m$ on an unknown input $x \in \{0,1\}^n$. The input $x$ can only be accessed by a unitary matrix $O_x$, called \textit{oracle}, that satisfies $O_x \ket{k}\ket{b} = \ket{k} \ket{b \oplus f(x)}$ for all $k \in \{1, \dots, n\}^n$ and $b \in \{0,1\}^m$, where $b \oplus f(x)$ denotes the bitwise XOR of $b$ and $f(x)$. Most of the provable and advantages of quantum algorithms over classical ones are in this model (for example, Grover's algorithm for search (\cite{grover1996fast}) and Shor's Algorithm for period finding (\cite{shor1999polynomial})) and this model is naturally connected to many other areas of quantum computing due to its simplicity. Thus, understanding the effects of noise in the query model is a natural question. 


\manaswicom{remove extensive, rephrase}
While there has been an extensive study on various types of noise in the query model, in this paper we only consider the situation when the oracle is affected by noise, referring the reader to~\cite{R03} for a survey for other types of noise types. There are two broad classes of noise models that one can consider: 
%that may affect the oracle: 
unitary (or reversible) and non-unitary (or irreversible). An example of reversible noisy oracle is a quantum circuit computing $f$ implemented on a fault-tolerant quantum quantum computer\footnote{talk about SAT}. \manaswicom{Is this okay? However, when such a circuit for $f$ is implemented on a quantum computer that is not fault-tolerant and is affected by noise do its interaction with the environment, we have an oracle for $f$ with non-reversible noise.}  It is known that the reversible noise is easy to mitigate: a quantum algorithm designed for a fault-less oracle with cost $T$ can be easily modified to give an algorithm for a with cost $O(T \log T)$ that works correctly on a oracle with reversible noise.\lauracom{Insert reference.}

The situation with non-reversible noise is much less clear \manaswicom{Say its hard} \manaswicom{Mention that its challenging to study: a specific algo is not hard but search is hard. Same for the next line.} and also more relevant today when we do not have large-scale fault tolerant quantum computers.
A majority of previous works study the effects of various types of non-reversible noise for the Grover algorithm~\cite{PR99, LLZT00, SBW03, FG98, ABNR12, KNR18} and more generally for the search problem~\cite{RS08, VRRW14, R03}. Generally speaking, these papers show that if noise occurs at a large enough rate\lauracom{When phrased this way, it seems obvious. Can we say somethign stronger, like that this already happens when noise is constant, independent of the system size. I think this is a realistic parameter regime. I don't expect anyone can build systems whose noise rate goes down with size. Rather the opposite. Would be good to make this point.}, then quantum advantage is lost for the search problem. We refer to~\cite{R03} for a survey of these results. A landmark \lauracom{Maybe too grand a word? What about Rosmanis' result?} result in this line of work was~\cite{RS08} which gave the first lower bound for the search problem under the following noise model: we are given access to an oracle $O_{f,p}$ which with probability $p$ fails and acts as identity, while with probability $(1-p)$ acts as $O_f$. The parameter $p$ is called the error-rate. This noise model, for the error-rate $p\leq 1/2$, is the central object of study in this paper. Following~\cite{RS08}, we refer to this error model as the \textit{faulty oracle} model.
% This noise model, specifically when $p = 1/2$, is the central object of study in this paper. 
\davidcom{This makes it seem like we can only handle error of $p=1/2$. We should probably make it clear that it can be easily extended to $p\le 1/2$.} \manaswicom{Sure. I wanted to stress that our results hold for constant $p$. I have changed the last line.}

\cite{RS08} showed an $\Omega(p2^n)$ lower bound for the search problem under the faulty oracle model. This lower bound has impacted several areas of research in quantum computing.~\cite{AGJMP15} considered quantum random access memory (qRAM) that stores classical information, i.e.~bits. Such a qRAM can be used as an oracle for quantum query algorithms.~\cite{AGJMP15} defines an error model which is quite similar to faulty oracle model. Using the lower bound from~\cite{RS08}, they showed that a qRAM that produces queries with constant error will not lead to quantum advantage for the search problem. Furthermore,~\cite{AGJMP15} conjectured that their error model nullifies the asymptotic speed-ups of other quantum query algorithms as well.~\cite{xu2023systems} emphasis that, in view of the lower bound of~\cite{RS08}, it is critical to guarantee the error robustness of qRAM, via either intrinsic noise resilience or error correction. Most supervised quantum machine learning algorithms assume existence of qRAM (\cite{GLM08}). In view of this and~\cite{RS08},~\cite{wossnig2021quantum} suggested that even small errors can crucially impact quantum machine learning algorithms.~\cite{R03} studies the query complexity of search problem under depolarizing noise, a more natural noise model, and gives an $\Omega(np)$ lower bound for the search problem under this noisy-oracle. \manaswicom{Write a few more refs in query complexity.}


While there is a large body of work that shows that quantum advantage is lost in the presence of noise, a natural question to ask is whether there are problems for which there is a quantum advantage even under a noisy oracle.
\lauracom{Can we sharpen the above? I think we need to differentiate between constant ``query depth'' and one that scales with problem size. In case of constant query depth, the speedup will probably be retained, e.g. as shown by Childs et al.}

\begin{center}
    \textit{\textbf{Question.}\cite{RS08, childs2023streaming} Is there any reasonable fault model under which a quantum speed-up is retained? Is a significant quantum speedup is ever possible with a faulty oracle?}
\end{center}


\manaswicom{Mention Simon's algorithm.}
If we restrict our attention to quantum algorithms where the (parallel) query depth is upper bounded by a constant, then the answer to the question is indeed yes (with a polynomial overhead) under the faulty oracle model.~\cite{childs2023streaming} studied the case when the oracle has dephasing noise. They showed that such quantum algorithms can be made robust with a polynomial overhead. However, their techniques do not extend to the algorithms that have $\omega(1)$ query depth without a substantial overhead. \manaswicom{Name the noise model as RS-Noisy Oracle? Define other noise models? TODO: Mention that we are dealing with constant error rate.}
\davidcom{So far I have called the noise for ``faulty oracle'', but I am not sure if there is a better name for it}
\lauracom{I think that somewhere on the first page we should already argue that in the context of noisy quantum computers, it is natural to consider the regime where the noise level is constant. So this is what we focus on.}

The main contribution of this paper is to show that \textit{any} quantum query algorithm can be made robust to the noise considered by~\cite{RS08} with a {\color{red}quadratic?} small polynomial overhead even when then error-rate $p = 1/2$ (given this, the case when $p < 1/2$ follows trivially). Thus we answer the \textbf{Question.} is affirmative for the extensively studied faulty oracle model for \textit{all} quantum algorithms that are sufficiently fast\footnote{Mention quantitatively}. In the next section, we describe our main results.

\section{Our Results}

We state our main theorem informally, referring to Section~\ref{} for the formal statement and a proof.
\lauracom{The theorem looks fully formal, no?}

\begin{theorem}[\textbf{Informal}]
\label{thm: Informal Main Theorem}
    Let $f : \cD \to \{0,1\}^m$, where $\cD \subseteq \{0,1\}^n$, such that there exists a quantum query algorithm that computes $f(x)$ for all $x \in \cD$ with probability at least $2/3$ while making at most $T$ queries to a fault-free oracle $O_f$. Then there exists a quantum algorithm that, given access to a faulty oracle $O_{f,p}$ with error-rate $p \leq 1/2$, computes $f(x)$ for all $x \in \cD$ with probability at least $2/3$ by making $O(T^3 m^2 \log T)$ many queries.
\end{theorem}

In particular, the query cost of a quantum algorithm for $f$ robust to noisy oracle is $O(Q(f)^3 \log Q(f))$, where $Q(f)$ is the quantum query complexity of $f$. Also note that it is natural to consider error-rate $p$ being smaller than $1/2$.

While quantum advantage is lost for the search problem with a faulty-oracle (\cite{RS08}), Theorem~\ref{thm: Informal Main Theorem} implies that a quantum advantage is retained for all problems for which there is a quantum algorithm with roughy super-cubic advantage. Furthermore, no additional structural assumptions are made about the algorithms, such as bounded-query depth as considered in~\cite{childs2023streaming}, in Theorem~\ref{thm: Informal Main Theorem}. Several quantum query algorithms that have super-cubic, super-polynomial and even exponential advantage over their classical counterparts. We refer the reader to~\cite{Zoo} which contains an extensive collection of such quantum algorithms.\manaswicom{Include some algorithms not in this list.} \manaswicom{Include some algorithms from property testing.}~\cite{RS08} asked the following question.

\begin{openproblem}[\cite{RS08}]
    Is there any search problem for which a quantum speed-up is achievable with a faulty oracle?
\end{openproblem}

Theorem~\ref{thm: Informal Main Theorem} resolves this problem in affirmative when combined with the following search algorithms: super-polynomial speedup for the welded tree problem which involves finding a special vertex in a certain graph (\cite{childs2003exponential, li2024recovering, jeffery2023multidimensional, belovs2024global})
and \textit{quartic} speedup for searching counterfeit coins given a bunch of coins (\cite{iwama2012quantum}). \manaswicom{Are there more?}

We conclude this section with some ideas that went into the proof of Theorem~\ref{thm: Informal Main Theorem}.



\manaswicom{Perhaps the theorems also hold for partial functions, i.e. functions with domain $D \subseteq \{0,1\}^n$. We could state the main theorem for such functions and say that the proof naturally extends to such functions. Writing in this manner is important as exponential quantum advantage is possible for partial functions.}

\manaswicom{Another nice thing to mention, if easily doable, is the blowup in the circuit size in the error-reduction in terms of the circuit size of the error free case.}

\manaswicom{For Boolean valued function $S$ is a one-qubit register. Do we add one qubit to $S$ each time we make query?}

\manaswicom{The circuit diagram of $F_f^t$ should have the register $B$ also? Since the oracle acts on $B$?}


